The Dichotomous Affiliate Stable Matching Problem: Approval-Based Matching with Applicant-Employer Relations

While the stable marriage problem and its variants model a vast range of matching markets, they fail to capture complex agent relationships, such as the affiliation of applicants and employers in an interview marketplace. To model this problem, the existing literature on matching with externalities permits agents to provide complete and total rankings over matchings based off of both their own and their affiliates' matches. This complete ordering restriction is unrealistic, and further the model may have an empty core. To address this, we introduce the Dichotomous Affiliate Stable Matching (DASM) Problem, where agents' preferences indicate dichotomous acceptance or rejection of another agent in the marketplace, both for themselves and their affiliates. We also assume the agent's preferences over entire matchings are determined by a general weighted valuation function of their (and their affiliates') matches. Our results are threefold: (1) we use a human study to show that real-world matching rankings follow our assumed valuation function; (2) we prove that there always exists a stable solution by providing an efficient, easily-implementable algorithm that finds such a solution; and (3) we experimentally validate the efficiency of our algorithm versus a linear-programming-based approach.

==> acks.tex <==

We thank Haris Aziz and Duncan McElfresh x  for comments on earlier versions of this work.
This research was supported in part by NSF CAREER Award IIS-1846237, NSF D-ISN Award \#2039862, NSF Award CCF-1852352, NIH R01 Award NLM-013039-01, NIST MSE Award \#20126334, DARPA GARD \#HR00112020007, and DoD WHS Award \#HQ003420F0035.

==> model_defn_old.tex <==
\section{Model Definition}\label{sec:model}
We now present our matching model.  
This model represents hiring markets where applicants have previous affiliations with employers and preferences are encoded as binary values that denote interest or disinterest (i.e., \emph{dichotomous preferences}~\citep{Bogomolnaia04:Random}). We describe the model in the most general many-to-many setting. We formalize the model (\S\ref{sec:model-prelims}), including defining valuation functions, stability, and other useful concepts (\S\ref{sec:model-defs}). We also introduce (\S\ref{sec:model-maximal}) the reserved maximal matching problem, which is a tool that we will use later (\S\ref{sec:theory}) in our algorithms.

\subsection{The \bamlong{} Problem}\label{sec:model-prelims}
In the \bamlong{} (\bam{}) Problem, we are given sets $A$ of $n$ applicants and $E$ of $m$ employers. For every $a\in A$ (resp. $e\in E$), we are given a complete preference function $\pr_a: E \to \{0,1\}$ (resp.\ $\pr_e^e:A\to \{0,1\}$, the notational difference will be clear later). If $u$ and $v$ are on opposite sides, then we say $u$ is \textit{interested} in or \textit{likes} $v$ if $\pr_u(v)=1$ (or $\pr_u^u(v)=1$ if $u\in E$), otherwise $u$ is \textit{disinterested} in or \textit{dislikes} $v$. The \textit{many-to-many} matching scenario specifies that $u$ might be matched with as many as $q(u)$ agents on the other side of the market, where $q(u)$ is the \textit{capacity} of $u$. A valid matching is a function $\mu:A\cup E \to 2^{A\cup E}$ such that for any $a\in A$ (resp. $e\in E$), $\mu(a) \subseteq E$ (resp. $\mu(e)\subseteq A$) and $|\mu(a)| \leq q(a)$ (resp. $|\mu(e)| \leq q(e)$), and $e\in \mu(a)$ if and only if $a\in \mu(e)$. %


One of the defining aspects of the dichotomous affiliate stable market is the notion of \textit{affiliates} which represent previous relationships between agents in the market. Let $\aff: E\to 2^A$ be the function that returns the set of affiliates for an employer. For instance, in Figure~\ref{fig:example}, $a_1$ is $e_1$'s affiliate, and $a_2$ and $a_3$ are both $e_2$'s affiliates. Then $\aff(e_1) = \{a_1\}$, $\aff(e_2) = \{a_2,a_3\}$, and $\aff(e_3)=\emptyset$. Note that $\aff$ over all $e\in E$ forms a disjoint cover of $A$, meaning that each applicant is the affiliate of exactly one employer. In this model, $e$ cares about where its affiliates are interviewed. To express this, for any $a\in \aff(e)$, $e$ has a preference function over potential matches for $a$: $\pr_e^a: E\to\{0,1\}$. To account for these preferences, $e$'s valuation of matches must be over tuples of its own matches \textit{and} its affiliates' matches. While these valuations may be general, we will examine a natural and flexible way to combine these two components for an employer to evaluate its preferences over entire matchings.

\begin{definition}
For any $e\in E$ and $a\in A$, we define the \textbf{weighted valuation function} over a match $\mu$ for a given weight $\lambda$ as:
\begin{align*}
\agg_e(\mu) =& \sum_{a^*\in \mu(e)} \pr_e^e(a^*) + \lambda\sum_{a_i\in\aff(e)} \sum_{e^*\in\mu(a_i)} \pr_e^{a_i}(e^*),
 \quad \quad \quad \val_a(\mu) =& \sum_{e^*\in\mu(a)} \pr_a(e^*).
\end{align*}
And we say $e$ or $a$ \textbf{prefers} $\mu$ to $\mu'$ ($\mu \succ_{e} \mu'$ or $\mu \succ_a \mu'$) if and only if $\agg_e(\mu) > \agg_e(\mu')$ or $\val_a(\mu) > \val_a(\mu')$.
\end{definition}

\input{example_fig}

We note that this function doesn't necessarily create a total order over matchings, as $e$ or $a$ may have the same valuation for two different matchings. Then it simply does not prefer one matching to another. In the employer variant of the valuation function, the regularization parameter $\lambda$ allows a user to define how employers weight the value of their affiliates' matches with respect to their own matches. If $\lambda=1$, then an employer cares about each individual match one of its affiliates has as much as each of its own matches. If $\lambda=0$, employers do not care about their affiliates' matches. To create a lexicographic valuation where employers care about their matches first and foremost and only use affiliates' matches as tiebreakers, then $\lambda$ should be set to some small $\epsilon>0$. To illustrate the role of $\lambda$, we discuss two stable marriages on the same example with respect to different $\lambda$ weights.

Consider again our example in Figure~\ref{fig:example} and let $\lambda=1$. Then $e_2$'s valuations of $\mu$ and $\mu'$ are: $\agg_{e_2}(\mu) = 3$ (since it likes one of its matches and both of its affiliates' matches) and $\agg_{e_2}(\mu') = 2$ (since it likes both of its matches). Therefore $\mu \succ_e \mu'$.

Now consider when $\lambda = \epsilon$. In this case, $e_2$'s valuations of the matchings are: $\afdef_{e_2}(\mu)  = 1 + 2\epsilon$ and $\afdef_{e_2}(\mu') = 2$. This means $\mu \prec_e \mu'$. This illustrates how changing $\lambda$ can change the stability of different matchings.



\subsection{Blocking Tuples, Stability, and Uniformity}\label{sec:model-defs}
Next, we define the notion of stability in the \bamprob{}. As in the standard stable marriage problem~\citep{Gale62:College} and its many variants, our notion of stability relies on the (non)existence of \emph{blocking tuples}.  The notion of a blocking tuple---traditionally, blocking \emph{pair}---is designed to identify a set of unmatched individuals who might break their own matches in order to match with each other. However, in our setting, agents are able to care about matches that do not directly involve them. At a high level, we would like to mitigate the following instability: {Some $a\in A$ and $e\in E$ can both improve their situation by (possibly) breaking matches to match with each other, and then allowing any abandoned agents to create any new match as long as all involved agents are interested and no other matches need to be broken.}

Without affiliations, this describes the stable marriage problem because $a$ and $e$ simply don't care about other matches being made. From $a$'s perspective, this holds even in the \bamprob{}: $a$ will only break a match to match with another agent if it improves their set of matches.

An employer $e$, however, may have additional reasons to deviate from a match. If they can somehow break their own match and rematch so that their affiliates have more favorable matches, they might do so even if it does not improve (or potentially worsens) their direct matches. For instance, if $a\in \aff(e)$, $e$ might be interested in breaking a match with $a'$ and matching with $a$ because it likes the match $(a,e)$ for $a$'s sake, not because it likes $a$ for itself. This relationship can get even more complicated if $a'\in\aff(e)$, or if $a$ breaks a match with some $e'$ who then matches with $a''$, where $a''\in\aff(e)$. There are additional complexities, too, that can impact if $e'$ decides to make a new match.

In the end, there are six agents that may be involved in a blocking tuple: $a$ and $e$ directly, their broken matches $e'$ and $a'$ respectively, and their ($e'$'s and $a'$'s) new matches $a''$ and $e''$ respectively. To understand our formal definition of the blocking tuple, it is useful to consider a \emph{potential blocking tuple}, which is simply a tuple such that, given a certain set of preferences, could form a blocking tuple.  Definition~\ref{def:potential-blocking-tuple} formalizes this concept, where we let $N_\mu^A$ (resp. $N_\mu^E$) be the applicants in $A$ (resp. employers in $E$) who have remaining quota under matching $\mu$.
Finally, we note that, in our many-to-many setting, there are some instances where $a$ and $e$ need not break their matches to form a blocking tuple. This corresponds to when they both have capacity to take on another match. To accommodate the sextuplet notation, we introduce the concept for a dummy or empty agent, $\gamma$ and its associated set $\mathcal{E}=\{\gamma\}$, which represents the absence of an agent.






\begin{definition}\label{def:potential-blocking-tuple}
A tuple $\T = (a,a',a'',e,e',e'')$ is a \textbf{potential blocking tuple} for a matching $\mu$ if all the following hold (where $\mathcal{E}$ is, again, the fake set of non-agents):
\begin{multicols}{2}
\begin{enumerate}
\item $a\in A$
\item $e\in E\setminus\mu(a)$
\item $a'\in \mu(e)\cup \mathcal{E}$
\item $e'\in \mu(a) \cup \mathcal{E}$
\item $a''\in (N_\mu^A\cup\mathcal{E}\cup\{a'\})\setminus\mu(e')$
\item $e''\in (N_\mu^A\cup \mathcal{E}\cup\{e'\})\setminus\mu(a')$. 
\end{enumerate}
\end{multicols}
Additionally, we require $a\in N_\mu^A$ if $e'\in\mathcal{E}$ and $e\in N_\mu^E$ if $a'\in \mathcal{E}$. Also, $a''\in\mathcal{E}$ if $e'\in\mathcal{E}$ and similarly $e''\in\mathcal{E}$ if $a'\in\mathcal{E}$. 
\end{definition}

We now clarify why we require each condition respectively:
\begin{enumerate}[itemsep=0mm]
\item $a$ must be an applicant
\item $e$ must be an employer that is not matched with $a$ (else they cannot form a blocking tuple)
\item $a'$ is $e$'s old match that is broken. If $e$ simply has additional capacity, then $a\in\mathcal{E}$ is a null agent.
\item $e'$ is $a$'s old match that is broken. If $a$ simply has additional capacity, then $e\in\mathcal{E}$ is a null agent.
\item $a''$ is $e'$'s new match. It must have unmatched capacity, or (if $e'$ and $a'$ decide to match) is instead $a'$ itself. It could be a null agent if $e'$ does not rematch. Additionally, we must ensure it was not previously matched to $e'$.
\item $e''$ is $a'$'s new match. It must have unmatched capacity, or (if $e'$ and $a'$ decide to match) is instead $e'$ itself. It could be a null agent if $a'$ does not rematch. Additionally, we must ensure it was not previously matched to $a'$.
\end{enumerate}


Let Figure \ref{fig:example} be a running example marketplace. Consider the tuple $ (a_3,a_2,a_2,e_2,e_1,e_1)$. Note that some agents are duplicated in this tuple; this is okay. This blocking tuple describes the following changes: (1) $a_3$ breaks its match with $e_1$, (2) $e_2$ breaks its match with $a_2$, (3) $a_3$ and $e_2$ match together, and (4) $a_2$ and $e_1$ match together. Note that the last part occurs explicitly because $a_2$ and $e_1$ appear twice in the tuple. If we rewrite the tuple as $ (a_3,a_2,a_2',e_2,e_1,e_1')$ to distinguish the instances of duplicates, then $a_2'$ indicates $e_1$ gets matched with $a_2$ and $e_1'$ indicates $a_2$ gets matched with $e_1$.

Note that, in this definition, we must add the matching constraints to ensure that old matches are properly broken and new matches can be made (i.e., no two agents will be matched to each other twice). When we consider a blocking tuple, we must compare the matching to the alternative matching that occurs after swapping as described.

\begin{definition}
Consider a potential blocking tuple comprising $\mathcal{T} = (a,a',a'',e,e',e'')$ and a matching $\mu$. Then matching $\mu'$ is the \textbf{swapped matching} of $\mu$ with respect to $\mathcal{T}$ if it can be formed by starting at $\mu$, breaking the matches $(a,e')$ and $(a',e)$, adding match $(a,e)$, and adding matches $(a',e'')$ and $(a'',e')$ if and only if those variables are not in $\mathcal{E}$ respectively.
\end{definition}


Note that this is a valid matching for the given instance. In Figure~\ref{fig:example}, $\mu'$ is the swapped matching of $\mu$ with respect to $(a_3, a_2, a_2, e_2, e_1, e_1)$.

\begin{prop}\label{prop:matching}
If $\mu$ is a valid matching, and $\mu'$ is the swapped matching of $\mu$ with respect to some potential blocking tuple $\mathcal{T}$, then $\mu'$ is a valid matching.
\end{prop}

Now we can define the blocking tuple.

\begin{definition}\label{def:block}
Consider a potential blocking tuple $\mathcal{T} = (a,a',a'',e,e',e'')$ for a matching $\mu$. Let $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$.  Then $\mathcal{T}$ is a \textbf{blocking tuple} under some valuation $f$ if all the following hold:
\begin{multicols}{2}
\begin{enumerate}
\item $\mu \prec_a \mu'$
\item $\mu \prec_e^f \mu'$
\item If $a'\notin\mathcal{E}$, then $\mu'\setminus\{(a',e'')\} \prec_{a'} \mu'$
\item If $e'\notin\mathcal{E}$, then $\mu'\setminus\{(a'',e')\} \prec_{e'}^f \mu'$
\item If $a''\notin\mathcal{E}$, then $\mu'\setminus\{(a'',e')\} \prec_{a''} \mu'$
\item If $e''\notin\mathcal{E}$, then $\mu'\setminus\{(a',e'')\} \prec_{e''}^f \mu'$
\end{enumerate}
\end{multicols}
\end{definition}

The first two conditions ensure that $a$ and $e$ (respectively) prefer the new match $\mu'$ to $\mu$. The next four state that in the context of $\mu'$, all of $a',e',a'',$ and $e''$ must have an active interest in forming the new match. In these conditions, we only care if $a'$, $a''$, $e'$, and $e''$ are not in $\mathcal{E}$ (i.e., they exist).

Consider again Figure~\ref{fig:example} when $\lambda=1$. Recall that $\T = (a_3, a_2, a_2, e_1, e_1)$ is a blocking tuple for $\mu$ and $\mu'$ is the swapped matching of $\mu$ with respect to $\T$. Under our weighted valuation function with $\lambda=1$, we already showed that $e_2$ prefers $\mu'$ to $\mu$. Additionally, since $a_3$ doesn't like its match in $\mu$ but likes its match in $\mu'$, it also prefers $\mu'$. Once $a_3$ and $e_2$ have broken their matches with $a_2$ and $e_1$ respectively, $a_2$ and $e_1$ have an active interest in matching. This implies that $\T$ satisfies all constraints in Definition~\ref{def:block} and is a blocking tuple. When $\lambda=\epsilon$ setting, since $e_2$ does not prefer $\mu'$ to $\mu$, this is not a blocking tuple.


\subsection{Reserved Maximal $b$-Matchings}\label{sec:model-maximal}

 The main result in Section \ref{sec:theory} is an algorithm for the \bamprob{}. It will require a subroutine that solves a new type of maximal matching problem. This is very closely related to a $b$-matching, but we define an affiliation between vertices and a \textit{reservation} on each affiliation (note: affiliations need not be disjoint). 

\begin{definition}\label{def:reservedmatch}
The \textbf{reserved maximal $b$-matching problem} is an instance of maximal $b$-matching with additional vertex subsets $S\subseteq V$ called \textbf{affiliations}, and each affiliation has a \textbf{reservation} number, designating how many vertices must \textit{not} be matched to their quota. A reserved maximal $b$-matching problem is represented as a graph $G=(V,E,q,\mathcal{S},r)$, where $V,E,$ and $q$ are the standard $b$-matching parameters, $\mathcal{S}\subseteq 2^V$ is the set of affiliations, and $r:\mathcal{S}\to\mathbb{N}$ is a reservation function such that $r(S) \leq |S|$ for all $S\in\mathcal{S}$.
\end{definition}

To clarify, consider an affiliation with 10 vertices, each with 100 capacity. The affiliation might have a reservation of 9 (of a max possible 10). We could then match each vertex in the affiliation 99 times, and one vertex 100 times. Then only one vertex has reached its quota, thus satisfying the reservation. One solution to this problem can be easily seen to be a simple greedy algorithm. 

\begin{prop}\label{prop:greedy-maximal-b-matching}
\textsf{Greedy} solves reserved maximal $b$-matching in $O(\left|E\right|)$ time for $E$ edges.
\end{prop}

Proposition~\ref{prop:greedy-maximal-b-matching} will be used in one of our main constructive theoretical results, Theorem~\ref{thm:match}, that gives a polynomial-time algorithm, Algorithm~\ref{alg:spm}, to solve variants of \bam{}.






==> pm_aggregated_proofs.tex <==
\subsection{Proofs for Section~\ref{sec:pm} (Aggregated Setting)}

We will use the following lemma many times throughout our proof so we state it here. The high level idea is that if we do a $\mu'$ is a swapped matching of $\mu$, agents only care about the part of their matches (and possibly their affiliate's matches) that change to decide which matching they like better. Specifically, we give conditions for an $a\in A$ and $e\in E$ where $a\notin\mu(e)$ but $a\in\mu'(e)$ would (weakly) \textit{not} prefer the new match to the old one. If this can be shown for all possible ways to do a pairwise swap to match $a$ and $e$, then they cannot form a blocking tuple. This is crucial to our proof.

\begin{lem}\label{lem:aggprefs}
Consider the aggregated stable market problem. Let $\mathcal{T} = (a,a',a'',b,b',b'')$ be a potential blocking tuple for a matching $\mu$, and $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$. Then both of the following hold:
\begin{enumerate}
\item If $\pr_a(e) \leq \pr_a(e')$, then $a$ cannot prefer $\mu'$ to $\mu$.
\item Let $I_a$, $I_{a'}$, and $I_{a''}$ be the respective indicators that $a,a',$ and $a''$ are in $\aff(e)$. Let $J_{a'',a'}$ be the indicator that $a''\neq a'$. If 
\begin{align*}
\pr_e^e(a)& + I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'') + I_{a''}J_{a'',a'}\pr_e^{a''}(e')\\&\leq \pr_e^e(a') + I_a\pr_e^a(e') + I_{a'} \pr_e^{a'}(e),
\end{align*}
then $e$ cannot prefer $\mu'$ to $\mu$.
\end{enumerate}
\end{lem}

\begin{proof}
For 1:
\begin{align*}
\agg_a(\mu') =& \pr_a(e) + \sum_{e^*\in \mu'(a)\setminus e} \pr_a(e^*)
\\\leq& \pr_a(e') + \sum_{e^*\in \mu(a)\setminus e'} \pr_a(e^*)\tag{1}\label{line:aggprefs1}
\\=&\agg_a(\mu),
\end{align*}
where line~\ref{line:aggprefs1} comes from the fact that the two summations sum over the same matches of $a$, and $\pr_a(e) \leq \pr_a(e')$. This completes the first part of the Lemma. We will now show 2, for $b_1,\ldots,b_{|\aff(a)|}\in\aff(a)$:
\begin{align*}
\agg_e&(\mu') \\=& \pr_e^e(a) + \sum_{a^*\in\mu'(e)\setminus\{a\}} \pr_e^e(a^*) + I_{a} \left(\pr_e^{a}(e) + \sum_{e^*\in\mu'(a)\setminus\{e\}} \pr_e^{a}(e^*)\right) 
\\&+ I_{a'} \left(\pr_e^{a'}(e'') + \sum_{e^*\in\mu'(a')\setminus\{e''\}} \pr_e^{a'}(e^*)\right) \\&+ I_{a''}J_{a'',a'} \left(\pr_e^{a''}(e') + \sum_{e^*\in\mu'(a'')\setminus\{e'\}} \pr_e^{a''}(e^*)\right) 
\\&+ \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in \mu'(a^*)} \pr_e^{a^*} (e^*)
\\\leq& \pr_e^e(a') + \sum_{a^*\in\mu(e)\setminus\{a'\}} \pr_e^e(a^*) + I_{a} \left(\pr_e^{a}(e') + \sum_{e^*\in\mu(a)\setminus\{e'\}} \pr_e^{a}(e^*)\right) 
\\&+ I_{a'} \left(\pr_e^{a'}(e) + \sum_{e^*\in\mu(a')\setminus\{e\}} \pr_e^{a'}(e^*)\right) \\&+ I_{a''}J_{a'',a'} \left(\sum_{e^*\in\mu(a'')} \pr_e^{a'}(e^*)\right) 
\\&+ \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in\mu(a^*)}\pr_e^{a^*} (e^*)\tag{2}\label{line:aggprefs2}
\\=& \agg_e(\mu)
\end{align*}
where line~\ref{line:aggprefs2} comes from the fact that all the summations are over the same matches, and otherwise the terms we pull out compose the provided inequality. When we pull out the summation for $a''$, note that this is only something we can pull out if $a''\neq a'$, because otherwise we already pulled it out as the $a'$ summation. This is why we scale it by $J_{a'',a'}$.
\end{proof}

We now introduce another useful lemma that implies that any potential blocking tuple with a nontrivial $a''$ cannot be a blocking tuple. Thus we can simplify the potential blocking tuples we consider to find blocking tuples.


\begin{lem}\label{lem:aggtup}
Let $\mu$ be the resulting matching from \textsf{PriorityMatch} in the aggregated setting. Then any blocking tuple $\T = (a,a',a'',e,e',e'')$ must satisfy $a'' = a'$ or $a'' \in \mathcal{E}$.
\end{lem}

\begin{proof}
Assume for contradiction there exists a blocking tuple where $a''\notin \mathcal{E}\cup \{a'\}$. Since $a$ prefers $\mu'$, Lemma~\ref{lem:aggprefs} implies that $\pr_a(e') = 0$. But since $(a,e')$ is a match, they must have been present in some graph. The only possible graph is $G_4$. Since they were both matched in $G_4$, that means $e'$ had unfilled quota in all previous matchings. Now we consider $a''$. Because this is a blocking tuple, we know $\mu'\setminus\{(a'',e')\} \prec_{a''} \mu'$ and $\mu'\setminus\{(a'',e')\} \prec_{e'}^f \mu'$. Obviously, this means $a''$ and $e'$ must both have an interest in $(a'',e')$: $\pr_{a''}(e') = 1 $ and either $\pr_{e'}^{e'}(a'')= 1$ or $a'' \in \aff(e')$ and $\pr_{e'}^{a''}(e') = 1$. In both cases, $(a'',e')$ appeared as an edge sometime before $G_4$. We already showed that $e'$ cannot have met its quota during the processing of the graph where $(a'',e')$ appears, and neither could $a''$ because it never meets its quota. Thus they should have been matched by \textsf{PriorityMatch}. This contradicts the definition of the blocking tuple.
\end{proof}



We now prove our main lemma of the section. Recall that in this setting, we run a maximal matching on $G_2\cup G_3$ instead of each of $G_2$ and $G_3$ independently. In this proof, we simply call that graph $G_2$. $G_4$ will still be the same, but we will not have a $G_3$.

\begin{proof}[Proof of Lemma~\ref{lem:agg}]
Obviously, as the quotas always reflect the maximum remaining space any agent has for  matches, this creates a valid matching. We show this is stable.

Assume for contradiction there is a blocking tuple for $\mu$, the output of \textsf{PriorityMatch} under the preconditions. By Lemma~\ref{lem:aggtup}, we can ignore the $a''$ parameter as it will either be the same as $e'$ or in $\mathcal{E}$. Thus our tuple is effectively reduced to $\mathcal{T} = (a,a',e,e',e'')$. Let $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$.

For $a$ and $e$ to form the blocking tuple, each must have some degree of interest $\mu'$ according to Lemma~\ref{lem:aggprefs}. This means $\pr_a(e) = 1$. For $e$, since it prefers $\mu'$, then at least one of the following must be true: $\pr_e^e(a)=1$, $a\in\aff(e)$ and $\pr_e^a(e)=1$, or $a'\in\aff(e)$ and $\pr_e^{a'}(e'')=1$. Note that when we refer to Lemma~\ref{lem:aggprefs}, we can ignore the $e''$ term because we know it will be zero by Lemma~\ref{lem:aggtup} (either $I_{a''} = 0$ or $J_{a'',a'}=0$).

Recall this Lemma has a precondition. To use it (as we will many times in the proof), we have to satisfy: $a,a'\in \aff(e)$ and $\mu \succ_a \mu'$. The latter is satisfied because we assume $\T$ is a blocking tuple. Therefore, we only have to show $a,a'\in\aff(a)$. Then we find:
\[\pr_e^e(a) + \pr_e^a(e) + \pr_e^{a'}(e'') \leq \pr_e^e(a') + \pr_e^a(e') + \pr_e^{a'}(e)\]

Since $I_a=I_{a'}=1$, this implies:

\[\pr_e^e(a) + I_a\pr_e^a(e) + I_{a'}\pr_e^{a'}(e'') \leq \pr_e^e(a') + I_{a}\pr_e^a(e') + I_{a'}\pr_e^{a'}(e)\]

Since we can ignore $e''$, this satisfies the second inequality of Lemma~\ref{lem:aggprefs}, which implies $e$ cannot prefer $\mu$ to $\mu'$ under aggregation. This is a contradiction. Therefore, any time we can prove $a,a'\in\aff(a)$, we immediately get a contradiction. 

\begin{enumerate}
\item\label{agg0} If $a\in\aff(e)$, $\pr_e^e(a) =1$, and $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_0$. Since it wasn't matched, that means $e$ must have reached its quota in $G_0$ without matching to $a$. That means $(a',e)$ was matched across by $\mu_0$, which implies that $a'\in\aff(e)$. Since $a,a'\in \aff(e)$, as stated previously, this yields a contradiction.


\item Else if $a\in\aff(e)$ and either $\pr_e^e(a) =1$ or $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_2$ (recall that in aggregation, $G_2$ and $G_3$ are unioned to get just one comprehensive graph $G_2$). Since they weren't matched, that means either $a$ or $e$ met its capacity beforehand, by $\mu_0$, $\mu_1$, or $\mu_2$. If it was $a$, then $a$ and $e'$ were matched in one of these matchings, so $\pr_a(e')=1$. Then by Lemma~\ref{lem:aggprefs}, $a$ cannot prefer $\mu'$. This is a contradiction.

Otherwise, we do an analysis of the right and lefthand sides of the 2nd Lemma~\ref{lem:aggprefs} inequality. We can assume $a'\notin\aff(e)$, otherwise we get our contradiction from $a,a'\in\aff(e)$. Thus $I_{a'}=0$. Then the left side of the inequality is:
\[\pr_e^e(a) + I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'') = 1 + 0 = 1\]
And on the right, note that since $e$ and $a'$ were matched in $\mu_0$, $\mu_1$, or $\mu_2$, then $\pr_e^e(a') = 1$ or $I_{a'}\pr_e^{a'}(e)=1$:
\[\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e) \geq 1 + I_a\pr_e^a(e') \geq 1\]
Clearly the second term is at least as large as the first, implying $e$ does not prefer $\mu'$ to $\mu$, a contradiction.

\item Else if $a\in \aff(e)$: At this point, $\pr_e^e(a)=0$ and $\pr_e^a(e)=0$. Again, we can assume $a'\notin\aff(e)$. Thus $e$ has nothing to gain from the matches formed in $\mu'$ (ie, the lefthand side of the second Lemma~\ref{lem:aggprefs} inequality is zero and thus it is satisfied), so we get our contradiction.


\item Else if $a' \in \aff(e)$, $\pr_e^e(a') = 1$, and $\pr_e^{a'}(e) = 1$: Then $\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e) = 2$. This is the righthand side of the 2nd inequality in Lemma~\ref{lem:aggprefs}. Since $e$ prefers $\mu'$, this must be less than the lefthand side. Therefore:
\[\pr_e^e(a) + I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'')  \geq 3\]
But since $I_a=0$, the maximum of this expression is 2. Thus we get a contradiction.
\item Else if $a'\in\aff(e)$ and either $\pr_e^e(a') = 1$ or $\pr_e^{a'}(e) = 1$: Then $(a',e)$ is an edge in $G_2$. That means $e$ could not have met its quota before $G_2$. Since $a$ and $e$ were not matched, either $a$ met its quota in or before $G_1$, or $(a,e)$ was not in $G_1$. The former is a contradiction because it would imply $\pr_a(e')=1$ because they were matched early, but $a$ prefers $\mu'$. The latter similarly implies $\pr_a(e)=0$, which would mean $a$ cannot prefer $\mu'$, or $e$ has no interest in $a$. This means that the lefthand side of our inequality will be at most 1, whereas the righthand side will be 1. Thus $a$ cannot prefer $\mu'$ to $\mu$.
\item Else if $a'\in \aff(e)$: At this point, $\pr_e^e(a') =0$ and $\pr_e^{a'}(e) = 0$. Thus $(a',e)$ could not have been in $G_0$, $G_1$, or $G_2$ because $e$ has no interest in $a'$. However, it cannot be in $G_4$ either since $a'\in\aff(e)$. This contradicts that $(a',e)$ were matched at all.
\item Else: Either $(a,e)$ is an edge in $G_1$, $\pr_a(e)=0$, or $\pr_e^e(a) = 0$. If $(a,e)$ is an edge in $G_1$, that means one of $a$ or $e$ was matched to their quota in $\mu_0$ or $\mu_1$. The former implies $\pr_a(e')=1$ because they were matched by $\mu_0$ or $\mu_1$, which is a contradiction. Otherwise, if it were $e$, then the only possibility is that $(a',e)$ was in $G_1$, which means, $\pr_e^e(a')=1$. So the righthand side of Lemma~\ref{lem:aggprefs} is $\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e)=1$. On the lefthand side, note that $I_a=I_{a'}=0$, so there is only one possibly nonzero term. Therefore, it clearly cannot be larger, implying $e$ prefers $\mu'$ to $\mu$. Next, note that $\pr_a(e) = 0$ is impossible because $a$ must prefer $\mu'$. Finally, consider when $\pr_e^e(a) = 0$. This implies the lefthand side of the 2nd inequality of Lemma~\ref{lem:aggprefs} is zero. Thus $e$ cannot prefer $\mu'$. In all cases, we get a contradiction.
\end{enumerate}
Thus we have contradicted the possibility of having a blocking tuple, so our algorithm produces a stable marriage.
\end{proof}


Finally, we prove the weakness of \textsf{PriorityMatch} in the prioritized setting.


\begin{proof}[Proof of Theorem~\ref{thm:bad} (Aggregated)]
Consider a market with two agents on each side: $A=\{a_1,a_2\}$ and $E=\{e_1,e_2\}$. We let $\aff(e_1) = \{a_1,a_2\}$ and $\aff(e_2) = \emptyset$. All possible preferences are set to one \textit{except} $\pr_{e_1}^{a_2}(e_2) = 0$, $\pr_{e_2}^{e_2}(a_2)=0$, and $\pr_{a_2}(e_2) = 0$. All quotas are 1. This means that $G_0$ contains edges $(a_1,e_1)$ and $(a_2,e_1)$. Since $e_1$ has a quota of 1, it must select only one edge. In an arbitrary maximal matching, it might select $(a_1,e_1)$. All other graphs, at this point, will either be empty, or only have edges with at least one 0-quota endpoint. Thus $a_2$ and $e_2$ will not be matched (though, we could imagine just arbitrarily matching the rest at the end and our argument will hold). However, note that $a_2$ likes $e_1$ and dislikes $e_2$. Similarly, $e_1$ would prefer for its affiliate $a_1$ to be matched with $e_2$ than $a_2$ be matched with $e_2$. Clearly, $a_2$ and $e_1$ would prefer to be matched and allow $a_1$ and $e_2$ to be matched. 
\end{proof}

==> pm_prioritized_proofs.tex <==
\subsection{Proofs for Section~\ref{sec:pm} (Affiliate-Deferential Setting)}

The proofs for the affiliate-deferential problem are quite similar to those of the aggregated problem. We start with a new lemma that addresses the same problem of qualifying when an agent prefers a new matching based off of a swap (as in the blocking pair).

\begin{lem}\label{lem:priorprefs}
Consider the affiliate-deferential stable market problem. Let $\mathcal{T} = (a,a',a'',e,e',e'')$ be a potential blocking tuple for a matching $\mu$, and $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$. Then both of the following hold:
\begin{enumerate}
\item If $\pr_a(e) \leq\pr_a(e')$, then $a$ cannot prefer $\mu'$ to $\mu$.
\item If $\pr_e^e(a) < \pr_e^e(b')$, then $e$ cannot prefer $\mu'$ to $\mu$.
\item Let $I_a$, $I_{a'}$, and $I_{a''}$ be the respective indicators that $a,a',$ and $a''$ are in $\aff(e)$. Let $J_{a'',a'}$ be the indicator that $a''\neq a'$. If $\pr_e^e(a)= \pr_e^e(a')$ and
\[I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'') + I_{a''}J_{a'',a'}\pr_e^{a''}(e')\leq I_a\pr_e^a(e') + I_{a'} \pr_e^{a'}(e)\]
then $e$ cannot prefer $\mu'$ to $\mu$.
\end{enumerate}
\end{lem}

\begin{proof}
The proof for (1) is exactly the same as the proof for (1) in $\ref{lem:aggprefs}$. We see that the math for (2) is similar as well:
\begin{align*}
\afdef_e^e(\mu') =& \pr_e^e(a) + \sum_{a^*\in \mu'(e)\setminus a} \pr_e^e(a^*)
\\\leq& \pr_e^e(a') + \sum_{a^*\in \mu(e)\setminus e} \pr_e(a^*)\tag{1}\label{line:priorprefs1}
\\=&\afdef_e^e(\mu),
\end{align*}
where line~\ref{line:priorprefs1} comes from the fact that the two summations sum over the same matches of $e$, and $\pr_e^e(a) \leq \pr_e^e(a')$. This completes the first part of the Lemma. We will now show (2):
\begin{align*}
\afdef_e^{\aff(e)}&(\mu') \\=& I_{a} \left(\pr_e^{a}(e) + \sum_{e^*\in\mu'(a)\setminus\{e\}} \pr_e^{a}(e^*)\right) 
\\&+ I_{a'} \left(\pr_e^{a'}(e'') + \sum_{e^*\in\mu'(a')\setminus\{e''\}} \pr_e^{a'}(e^*)\right) \\&+ I_{a''}J_{a'',a'} \left(\pr_e^{a''}(e') + \sum_{e^*\in\mu'(a'')\setminus\{e'\}} \pr_e^{a''}(e^*)\right) 
\\&+ \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in \mu'(a^*)} \pr_e^{a^*} (e^*)
\\\leq&  I_{a} \left(\pr_e^{a}(e') + \sum_{e^*\in\mu(a)\setminus\{e'\}} \pr_e^{a}(e^*)\right) 
\\&+ I_{a'} \left(\pr_e^{a'}(e) + \sum_{e^*\in\mu(a')\setminus\{e\}} \pr_e^{a'}(e^*)\right) \\&+ I_{a''}J_{a'',a'} \left(\sum_{e^*\in\mu(a'')} \pr_e^{a'}(e^*)\right) 
\\&+ \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in\mu(a^*)}\pr_e^{a^*} (e^*)\tag{2}\label{line:priorprefs2}
\\=& \afdef_e^{\aff(e)}(\mu)
\end{align*}
where line~\ref{line:priorprefs2} comes from the fact that all the summations are over the same matches, and otherwise the terms we pull out compose the provided inequality. When we pull out the summation for $a''$, note that this is only something we can pull out if $a''\neq a'$, because otherwise we already pulled it out as the $a'$ summation. This is why we scale it by $J_{a'',a'}$.
\end{proof}

Our second helper lemma will again be quite similar to the aggregated case.

\begin{lem}\label{lem:priortup}
Let $\mu$ be the resulting matching from \textsf{PriorityMatch} in the prioritized setting. Then any blocking tuple must have $a'' = a'$ or $a'' \in \mathcal{E}$.
\end{lem}

\begin{proof}
The proof here is the same as that of Lemma~\ref{lem:aggtup}, but instead of referring to Lemma~\ref{lem:aggprefs}, we use Lemma~\ref{lem:priorprefs}.
\end{proof}

We now prove our lemma. This proof will also follow a very similar flow to the proof in the aggregated context.

\begin{proof}[Proof of Lemma~\ref{lem:prior}]
Obviously, as the quotas always reflect the maximum remaining space any agent has for  matches, this creates a valid matching. We show this is stable.

Assume for contradiction there is a blocking tuple for $\mu$, the output of \textsf{PriorityMatch} under the preconditions. By Lemma~\ref{lem:priortup}, we can ignore the $a''$ parameter as it will either be the same as $e'$ or in $\mathcal{E}$. Thus our tuple is effectively reduced to $\mathcal{T} = (a,a',e,e',e'')$. Let $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$.

For $a$ and $e$ to form the blocking tuple, each must have some degree of interest $\mu'$ according to Lemma~\ref{lem:priorprefs}. This means $\pr_a(e) = 1$. For $e$, since it prefers $\mu'$, then at least one of the following must be true: $\pr_e^e(a)=1$, $a\in\aff(e)$ and $\pr_e^a(e)=1$, or $a'\in\aff(e)$ and $\pr_e^{a'}(e'')=1$. Note that when we refer to Lemma~\ref{lem:priorprefs}, we can ignore the $e''$ term because we know it will be zero by Lemma~\ref{lem:priortup} (either $I_{a''} = 0$ or $J_{a'',a'}=0$).

Recall this Lemma has a precondition. To use it (as we will many times in the proof), we have to satisfy: $a,a'\in \aff(e)$ and $\mu \succ_a \mu'$. The latter is satisfied because we assume $\T$ is a blocking tuple. Therefore, we only have to show $a,a'\in\aff(a)$. Then we find:
\[\pr_e^a(e) + \pr_e^{a'}(e'') \leq \pr_e^a(e') + \pr_e^{a'}(e)\]

Since $I_a=I_{a'}=1$, this implies:

\[I_a\pr_e^a(e) + I_{a'}\pr_e^{a'}(e'') \leq I_{a}\pr_e^a(e') + I_{a'}\pr_e^{a'}(e)\]

Since we can ignore $e''$, this satisfies the second inequality of Lemma~\ref{lem:priorprefs}, which implies $e$ cannot prefer $\mu$ to $\mu'$ under aggregation. This is a contradiction. Therefore, any time we can prove $a,a'\in\aff(a)$, we immediately get a contradiction. 

\begin{enumerate}
\item\label{agg0} If $a\in\aff(e)$, $\pr_e^e(a) =1$, and $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_0$. Since it wasn't matched, that means $e$ must have reached its quota in $G_0$ without matching to $a$. That means $(a',e)$ was matched across by $\mu_0$, which implies that $a'\in\aff(e)$. Since $a,a'\in \aff(e)$, as stated previously, this yields a contradiction.


\item Else if $a\in\aff(e)$ and $\pr_e^e(a) =1$: Then $(a,e)$ is an edge in $G_2$. Since they weren't matched, that means either $a$ or $e$ met its capacity beforehand, by $\mu_0$, $\mu_1$, or $\mu_2$. If it was $a$, then $a$ and $e'$ were matched in one of these matchings, so $\pr_a(e')=1$. Then by Lemma~\ref{lem:priorprefs}, $a$ cannot prefer $\mu'$. This is a contradiction.

Otherwise, we do an analysis of the right and lefthand sides of the 3rd Lemma~\ref{lem:priorprefs} inequality. We can assume $a'\notin\aff(e)$, otherwise we get our contradiction from $a,a'\in\aff(e)$. Thus $I_{a'}=0$. We also know that in this case $\pr_e^a(e)=0$. Therefore
\[I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'') = 0\]
Since this is the minimum value for the righthand side of the inequality, we know the inequality is satisfied. Thus $e$ does not prefer $\mu$ to $\mu'$, a contradiction.

\item Else if $a\in\aff(e)$ and $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_3$. Since they weren't matched, that means either $a$ or $e$ met its capacity beforehand, by $\mu_0$, $\mu_1$, $\mu_2$, or $\mu_3$. If it was $a$, then $a$ and $e'$ were matched in one of these matchings, so $\pr_a(e')=1$. Then by Lemma~\ref{lem:priorprefs}, $a$ cannot prefer $\mu'$. This is a contradiction.

Otherwise, we do an analysis of the right and lefthand sides of the 3rd Lemma~\ref{lem:priorprefs} inequality. We can assume $a'\notin\aff(e)$, otherwise we get our contradiction from $a,a'\in\aff(e)$. Thus $I_{a'}=0$. If $(a', e)$ were matched in $\mu_0$, $\mu_1$, or $\mu_2$, then $\pr_e^e(a')=1$, which means $\pr_e^e(a)=0 < \pr_e^e(a')$ so the 2nd inequality of Lemma~\ref{lem:priorprefs} implies the contradiction. Otherwise,$\pr_e^e(a) = \pr_e^e(a') = 0$. Also $(a,e')$ were matched in $\mu_3$, so $\pr_e^{a'}(e) = 1$. Then the left side of the inequality is:
\[I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'') = 1 + 0 = 1\]
And on the right side:
\[\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e) \geq 1 + I_a\pr_e^a(e') \geq 1\]
Clearly the second term is at least as large as the first, implying $e$ does not prefer $\mu'$ to $\mu$, a contradiction.

\item Else if $a\in \aff(e)$: At this point, $\pr_e^e(a)=0$ and $\pr_e^a(e)=0$. Again, we can assume $a'\notin\aff(e)$. Thus $e$ has nothing to gain from the matches formed in $\mu'$ (ie, the lefthand side of the second Lemma~\ref{lem:priorprefs} inequality is zero and thus it is satisfied), so we get our contradiction.


\item Else if $a' \in \aff(e)$, $\pr_e^e(a') = 1$, and $\pr_e^{a'}(e) = 1$: Then $\pr_e^e(a') \geq \pr_e^e(a)$, so either $\pr_e^e(a') > \pr_e^e(a)$ and we immediately get our contradiction from the 2nd inequality of Lemma~\ref{lem:aggprefs}, or $\pr_e^e(a') = \pr_e^e(a)$. In this case, we additionally have $I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e) = 1$. This is the righthand side of the 2nd inequality in Lemma~\ref{lem:aggprefs}. Since $e$ prefers $\mu'$, this must be less than the lefthand side. Therefore:
\[ I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'')  \geq 2\]
But since $I_a=0$, the maximum of this expression is 1. Thus we get a contradiction.

\item Else if $a'\in\aff(e)$ and $\pr_e^e(a') = 1$: Then $(a',e)$ is an edge in $G_2$. That means $e$ could not have met its quota before $G_2$. Since $a$ and $e$ were not matched, either $a$ met its quota in or before $G_1$, or $(a,e)$ was not in $G_1$. The former is a contradiction because it would imply $\pr_a(e')=1$ because they were matched early, but $a$ prefers $\mu'$. The latter similarly implies $\pr_a(e)=0$, which would mean $a$ cannot prefer $\mu'$, or $e$ has no interest in $a$, so $\pr_e^e(a)=0$. Thus $\pr_e^e(a) < \pr_e^e(a')$, so by the 2nd inequality and Lemma~\ref{lem:priorprefs} implies $e$ cannot prefer $\mu'$ to $\mu$.

\item Else if $a'\in\aff(e)$ and $\pr_e^{a'}(e) = 1$: Then $(a',e)$ is an edge in $G_3$. That means $e$ could not have met its quota before $G_3$. Since $a$ and $e$ were not matched, either $a$ met its quota in or before $G_1$, or $(a,e)$ was not in $G_1$. The former is a contradiction from the same explanation as before. The latter implies $\pr_a(e)=0$, which again reaches a contradiction, or $e$ has no interest in $a$. This means that $\pr_e^e(a) = 0 = \pr_e^e(a')$. The lefthand side of the third inequality will be at most 1, whereas the righthand side will be 1. Thus $a$ cannot prefer $\mu'$ to $\mu$.

\item Else if $a'\in \aff(e)$: At this point, $\pr_e^e(a') =0$ and $\pr_e^{a'}(e) = 0$. Thus $(a',e)$ could not have been in $G_0$, $G_1$, or $G_2$ because $e$ has no interest in $a'$. However, it cannot be in $G_4$ either since $a'\in\aff(e)$. This contradicts that $(a',e)$ were matched at all.

\item Else: Either $(a,e)$ is an edge in $G_1$, $\pr_a(e)=0$, or $\pr_e^e(a) = 0$. If $(a,e)$ is an edge in $G_1$, that means one of $a$ or $e$ was matched to their quota in $\mu_0$ or $\mu_1$. The former implies $\pr_a(e')=1$ because they were matched by $\mu_0$ or $\mu_1$, which is a contradiction. Otherwise, if it were $e$, then the only possibility is that $(a',e)$ was in $G_1$, which means, $\pr_e^e(a')=1$. So either $\pr_e^e(a') > \pr_e^e(a)$, which immediately give sthe contradiction, or $\pr_e^e(a')=\pr_e^e(a)$. For the 3rd inequality of Lemma~\ref{lem:priorprefs}, since $I_a=I_{a'}=0$, both sides are 0, meaning the equality holds. This gives us the contradiction. Next, note that $\pr_a(e) = 0$ is impossible because $a$ must prefer $\mu'$. Finally, consider when $\pr_e^e(a) = 0$. This implies the lefthand side of the 2nd inequality of Lemma~\ref{lem:aggprefs} is zero. Thus $e$ cannot prefer $\mu'$. In all cases, we get a contradiction.
\end{enumerate}
Thus we have contradicted the possibility of having a blocking tuple, so our algorithm produces a stable marriage.
\end{proof}

Finally, we prove the weakness of \textsf{PriorityMatch} in the affiliate-deferential setting.


\begin{proof}[Proof of Theorem~\ref{thm:bad} (Prioritized)]
The example is the same as in the aggregated settings. It is not hard to see that $a_1$ and $b_2$ would still prefer to match and allow $b_1$ and $a_2$ to match.
\end{proof}

==> proofs.tex <==
\subsection{Proofs for Section~\ref{sec:theory}}

In this section, we present the proofs for our theoretical work. To start, we introduce a new lemma that will simply show a useful property that we use throughout the proofs. The high level idea is that if matching $\mu'$ is a swapped matching of $\mu$, agents only care about the part of their matches (and possibly their affiliate's matches) that change to decide which matching they like better. Specifically, we give conditions for an $a\in A$ and $e\in E$ where $a\notin\mu(e)$ but $a\in\mu'(e)$ would (weakly) \textit{not} prefer the new match to the old one. If this can be shown for all possible ways to do a pairwise swap to match $a$ and $e$, then they cannot form a blocking tuple. This is crucial to our proof.

\begin{lem}\label{lem:prefs}
Consider the \bamprob{}. Let $\mathcal{T} = (a,a',a'',b,b',b'')$ be a potential blocking tuple for a matching $\mu$, and $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$. Then both of the following hold:
\begin{enumerate}
\item If $\pr_a(e) \leq \pr_a(e')$, then $a$ cannot prefer $\mu'$ to $\mu$.
\item Let $I_a$, $I_{a'}$, and $I_{a''}$ be the respective indicators that $a,a',$ and $a''$ are in $\aff(e)$. Let $J_{a'',a'}$ be the indicator that $a''\neq a'$. If 
\begin{align*}
\pr_e^e(a)& + \lambda I_a\pr_e^{a}(e) + \lambda I_{a'}\pr_e^{a'}(e'') + \lambda I_{a''}J_{a'',a'}\pr_e^{a''}(e')\\&\leq \pr_e^e(a') + \lambda I_a\pr_e^a(e') + \lambda I_{a'} \pr_e^{a'}(e),
\end{align*}
then $e$ cannot prefer $\mu'$ to $\mu$.
\end{enumerate}
\end{lem}

\begin{proof}
For 1:
\begin{align*}
\agg_a(\mu') =& \pr_a(e) + \sum_{e^*\in \mu'(a)\setminus e} \pr_a(e^*)
\\\leq& \pr_a(e') + \sum_{e^*\in \mu(a)\setminus e'} \pr_a(e^*)\tag{1}\label{line:prefs1}
\\=&\agg_a(\mu),
\end{align*}
where line~\ref{line:prefs1} comes from the fact that the two summations sum over the same matches of $a$, and $\pr_a(e) \leq \pr_a(e')$. This completes the first part of the Lemma. We will now show 2, for $b_1,\ldots,b_{|\aff(a)|}\in\aff(a)$:
\begin{align*}
\agg_e&(\mu') \\=& \pr_e^e(a) + \sum_{a^*\in\mu'(e)\setminus\{a\}} \pr_e^e(a^*) + \lambda I_{a} \left(\pr_e^{a}(e) + \sum_{e^*\in\mu'(a)\setminus\{e\}} \pr_e^{a}(e^*)\right) 
\\&+ \lambda I_{a'} \left(\pr_e^{a'}(e'') + \sum_{e^*\in\mu'(a')\setminus\{e''\}} \pr_e^{a'}(e^*)\right) \\&+\lambda  I_{a''}J_{a'',a'} \left(\pr_e^{a''}(e') + \sum_{e^*\in\mu'(a'')\setminus\{e'\}} \pr_e^{a''}(e^*)\right) 
\\&+ \lambda \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in \mu'(a^*)} \pr_e^{a^*} (e^*)
\\\leq& \pr_e^e(a') + \sum_{a^*\in\mu(e)\setminus\{a'\}} \pr_e^e(a^*) + \lambda I_{a} \left(\pr_e^{a}(e') + \sum_{e^*\in\mu(a)\setminus\{e'\}} \pr_e^{a}(e^*)\right) 
\\&+ \lambda I_{a'} \left(\pr_e^{a'}(e) + \sum_{e^*\in\mu(a')\setminus\{e\}} \pr_e^{a'}(e^*)\right) \\&+\lambda  I_{a''}J_{a'',a'} \left(\sum_{e^*\in\mu(a'')} \pr_e^{a'}(e^*)\right) 
\\&+ \lambda \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in\mu(a^*)}\pr_e^{a^*} (e^*)\tag{2}\label{line:prefs2}
\\=& \agg_e(\mu)
\end{align*}
where line~\ref{line:prefs2} comes from the fact that all the summations are over the same matches, and otherwise the terms we pull out compose the provided inequality. When we pull out the summation for $a''$, note that this is only something we can pull out if $a''\neq a'$, because otherwise we already pulled it out as the $a'$ summation. This is why we scale it by $J_{a'',a'}$.
\end{proof}

We now introduce another useful lemma that implies that any potential blocking tuple with a nontrivial $a''$ cannot be a blocking tuple. Thus we can simplify the potential blocking tuples we consider to find blocking tuples.


\begin{lem}\label{lem:aggtup}
Let $\mu$ be the resulting matching from \textsf{PriorityMatch}. Then any blocking tuple $\T = (a,a',a'',e,e',e'')$ must satisfy $a'' = a'$ or $a'' \in \mathcal{E}$.
\end{lem}

\begin{proof}
Assume for contradiction there exists a blocking tuple $\mathcal{T} = (a,a',a'',e,e',e'')$ where $a''\notin \mathcal{E}\cup \{a'\}$. Let $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$. Then both $a$ and $e$ must prefer $\mu'$ to $\mu$. Since $a$ prefers $\mu'$, Lemma~\ref{lem:prefs} implies that $\pr_a(e') = 0$. But since $e'\in\mu(a)$, the edge $(a,e')$ must have been present in some graph during the execution of \prm. I AM HERE NEED TO CHANGE GRAPH LABELS The only possible graph is $G_3$. Since they were both matched in $G_3$, that means $e'$ had unfilled quota in all previous matchings. Now we consider $a''$. Because this is a blocking tuple, we know $\mu'\setminus\{(a'',e')\} \prec_{a''} \mu'$ and $\mu'\setminus\{(a'',e')\} \prec_{e'}^f \mu'$. Obviously, this means $a''$ and $e'$ must both have an interest in $(a'',e')$: $\pr_{a''}(e') = 1 $ and either $\pr_{e'}^{e'}(a'')= 1$ or $a'' \in \aff(e')$ and $\pr_{e'}^{a''}(e') = 1$. In both cases, $(a'',e')$ appeared as an edge sometime before $G_4$. We already showed that $e'$ cannot have met its quota during the processing of the graph where $(a'',e')$ appears, and neither could $a''$ because it never meets its quota. Thus they should have been matched by \textsf{PriorityMatch}. This contradicts the definition of the blocking tuple.
\end{proof}



We now prove our main lemma of the section. Recall that in this setting, we run a maximal matching on $G_2\cup G_3$ instead of each of $G_2$ and $G_3$ independently. In this proof, we simply call that graph $G_2$. $G_4$ will still be the same, but we will not have a $G_3$.

\begin{proof}[Proof of Lemma~\ref{lem:agg}]
Obviously, as the quotas always reflect the maximum remaining space any agent has for  matches, this creates a valid matching. We show this is stable.

Assume for contradiction there is a blocking tuple for $\mu$, the output of \textsf{PriorityMatch} under the preconditions. By Lemma~\ref{lem:aggtup}, we can ignore the $a''$ parameter as it will either be the same as $e'$ or in $\mathcal{E}$. Thus our tuple is effectively reduced to $\mathcal{T} = (a,a',e,e',e'')$. Let $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$.

For $a$ and $e$ to form the blocking tuple, each must have some degree of interest $\mu'$ according to Lemma~\ref{lem:aggprefs}. This means $\pr_a(e) = 1$. For $e$, since it prefers $\mu'$, then at least one of the following must be true: $\pr_e^e(a)=1$, $a\in\aff(e)$ and $\pr_e^a(e)=1$, or $a'\in\aff(e)$ and $\pr_e^{a'}(e'')=1$. Note that when we refer to Lemma~\ref{lem:aggprefs}, we can ignore the $e''$ term because we know it will be zero by Lemma~\ref{lem:aggtup} (either $I_{a''} = 0$ or $J_{a'',a'}=0$).

Recall this Lemma has a precondition. To use it (as we will many times in the proof), we have to satisfy: $a,a'\in \aff(e)$ and $\mu \succ_a \mu'$. The latter is satisfied because we assume $\T$ is a blocking tuple. Therefore, we only have to show $a,a'\in\aff(a)$. Then we find:
\[\pr_e^e(a) + \pr_e^a(e) + \pr_e^{a'}(e'') \leq \pr_e^e(a') + \pr_e^a(e') + \pr_e^{a'}(e)\]

Since $I_a=I_{a'}=1$, this implies:

\[\pr_e^e(a) + I_a\pr_e^a(e) + I_{a'}\pr_e^{a'}(e'') \leq \pr_e^e(a') + I_{a}\pr_e^a(e') + I_{a'}\pr_e^{a'}(e)\]

Since we can ignore $e''$, this satisfies the second inequality of Lemma~\ref{lem:aggprefs}, which implies $e$ cannot prefer $\mu$ to $\mu'$ under aggregation. This is a contradiction. Therefore, any time we can prove $a,a'\in\aff(a)$, we immediately get a contradiction. 

\begin{enumerate}
\item\label{agg0} If $a\in\aff(e)$, $\pr_e^e(a) =1$, and $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_0$. Since it wasn't matched, that means $e$ must have reached its quota in $G_0$ without matching to $a$. That means $(a',e)$ was matched across by $\mu_0$, which implies that $a'\in\aff(e)$. Since $a,a'\in \aff(e)$, as stated previously, this yields a contradiction.


\item Else if $a\in\aff(e)$ and either $\pr_e^e(a) =1$ or $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_2$ (recall that in aggregation, $G_2$ and $G_3$ are unioned to get just one comprehensive graph $G_2$). Since they weren't matched, that means either $a$ or $e$ met its capacity beforehand, by $\mu_0$, $\mu_1$, or $\mu_2$. If it was $a$, then $a$ and $e'$ were matched in one of these matchings, so $\pr_a(e')=1$. Then by Lemma~\ref{lem:aggprefs}, $a$ cannot prefer $\mu'$. This is a contradiction.

Otherwise, we do an analysis of the right and lefthand sides of the 2nd Lemma~\ref{lem:aggprefs} inequality. We can assume $a'\notin\aff(e)$, otherwise we get our contradiction from $a,a'\in\aff(e)$. Thus $I_{a'}=0$. Then the left side of the inequality is:
\[\pr_e^e(a) + I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'') = 1 + 0 = 1\]
And on the right, note that since $e$ and $a'$ were matched in $\mu_0$, $\mu_1$, or $\mu_2$, then $\pr_e^e(a') = 1$ or $I_{a'}\pr_e^{a'}(e)=1$:
\[\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e) \geq 1 + I_a\pr_e^a(e') \geq 1\]
Clearly the second term is at least as large as the first, implying $e$ does not prefer $\mu'$ to $\mu$, a contradiction.

\item Else if $a\in \aff(e)$: At this point, $\pr_e^e(a)=0$ and $\pr_e^a(e)=0$. Again, we can assume $a'\notin\aff(e)$. Thus $e$ has nothing to gain from the matches formed in $\mu'$ (ie, the lefthand side of the second Lemma~\ref{lem:aggprefs} inequality is zero and thus it is satisfied), so we get our contradiction.


\item Else if $a' \in \aff(e)$, $\pr_e^e(a') = 1$, and $\pr_e^{a'}(e) = 1$: Then $\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e) = 2$. This is the righthand side of the 2nd inequality in Lemma~\ref{lem:aggprefs}. Since $e$ prefers $\mu'$, this must be less than the lefthand side. Therefore:
\[\pr_e^e(a) + I_a\pr_e^{a}(e) + I_{a'}\pr_e^{a'}(e'')  \geq 3\]
But since $I_a=0$, the maximum of this expression is 2. Thus we get a contradiction.
\item Else if $a'\in\aff(e)$ and either $\pr_e^e(a') = 1$ or $\pr_e^{a'}(e) = 1$: Then $(a',e)$ is an edge in $G_2$. That means $e$ could not have met its quota before $G_2$. Since $a$ and $e$ were not matched, either $a$ met its quota in or before $G_1$, or $(a,e)$ was not in $G_1$. The former is a contradiction because it would imply $\pr_a(e')=1$ because they were matched early, but $a$ prefers $\mu'$. The latter similarly implies $\pr_a(e)=0$, which would mean $a$ cannot prefer $\mu'$, or $e$ has no interest in $a$. This means that the lefthand side of our inequality will be at most 1, whereas the righthand side will be 1. Thus $a$ cannot prefer $\mu'$ to $\mu$.
\item Else if $a'\in \aff(e)$: At this point, $\pr_e^e(a') =0$ and $\pr_e^{a'}(e) = 0$. Thus $(a',e)$ could not have been in $G_0$, $G_1$, or $G_2$ because $e$ has no interest in $a'$. However, it cannot be in $G_4$ either since $a'\in\aff(e)$. This contradicts that $(a',e)$ were matched at all.
\item Else: Either $(a,e)$ is an edge in $G_1$, $\pr_a(e)=0$, or $\pr_e^e(a) = 0$. If $(a,e)$ is an edge in $G_1$, that means one of $a$ or $e$ was matched to their quota in $\mu_0$ or $\mu_1$. The former implies $\pr_a(e')=1$ because they were matched by $\mu_0$ or $\mu_1$, which is a contradiction. Otherwise, if it were $e$, then the only possibility is that $(a',e)$ was in $G_1$, which means, $\pr_e^e(a')=1$. So the righthand side of Lemma~\ref{lem:aggprefs} is $\pr_e^e(a') + I_a\pr_e^a(e') + I_{a'}\pr_e^{a'}(e)=1$. On the lefthand side, note that $I_a=I_{a'}=0$, so there is only one possibly nonzero term. Therefore, it clearly cannot be larger, implying $e$ prefers $\mu'$ to $\mu$. Next, note that $\pr_a(e) = 0$ is impossible because $a$ must prefer $\mu'$. Finally, consider when $\pr_e^e(a) = 0$. This implies the lefthand side of the 2nd inequality of Lemma~\ref{lem:aggprefs} is zero. Thus $e$ cannot prefer $\mu'$. In all cases, we get a contradiction.
\end{enumerate}
Thus we have contradicted the possibility of having a blocking tuple, so our algorithm produces a stable marriage.
\end{proof}


Finally, we prove the weakness of \textsf{PriorityMatch} in the prioritized setting.


\begin{proof}[Proof of Theorem~\ref{thm:bad} (Aggregated)]
Consider a market with two agents on each side: $A=\{a_1,a_2\}$ and $E=\{e_1,e_2\}$. We let $\aff(e_1) = \{a_1,a_2\}$ and $\aff(e_2) = \emptyset$. All possible preferences are set to one \textit{except} $\pr_{e_1}^{a_2}(e_2) = 0$, $\pr_{e_2}^{e_2}(a_2)=0$, and $\pr_{a_2}(e_2) = 0$. All quotas are 1. This means that $G_0$ contains edges $(a_1,e_1)$ and $(a_2,e_1)$. Since $e_1$ has a quota of 1, it must select only one edge. In an arbitrary maximal matching, it might select $(a_1,e_1)$. All other graphs, at this point, will either be empty, or only have edges with at least one 0-quota endpoint. Thus $a_2$ and $e_2$ will not be matched (though, we could imagine just arbitrarily matching the rest at the end and our argument will hold). However, note that $a_2$ likes $e_1$ and dislikes $e_2$. Similarly, $e_1$ would prefer for its affiliate $a_1$ to be matched with $e_2$ than $a_2$ be matched with $e_2$. Clearly, $a_2$ and $e_1$ would prefer to be matched and allow $a_1$ and $e_2$ to be matched. 
\end{proof}

==> proofs2.tex <==
\section{Proofs for Section~\ref{sec:theory}}

In this section, we present the proofs for our theoretical work. To start, we introduce a new lemma that will simply show a useful property that we use throughout the proofs. The high level idea is that if matching $\mu'$ is a swapped matching of $\mu$, agents only care about the part of their matches (and possibly their affiliate's matches) that change to decide which matching they like better. Specifically, we give conditions for an $a\in A$ and $e\in E$ where $a\notin\mu(e)$ but $a\in\mu'(e)$ would (weakly) \textit{not} prefer the new match to the old one. If this can be shown for all possible ways to do a pairwise swap to match $a$ and $e$, then they cannot form a blocking tuple. This is crucial to our proof.

\begin{lem}\label{lem:prefs}
Consider the \bamprob{}. Let $\mathcal{T} = (a,a',a'',b,b',b'')$ be a potential blocking tuple for a matching $\mu$, and $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$. Then both of the following hold:
\begin{enumerate}
\item If $\pr_a(e) \leq \pr_a(e')$, then $a$ cannot prefer $\mu'$ to $\mu$.
\item Let $I_a$, $I_{a'}$, and $I_{a''}$ be the respective indicators that $a,a',$ and $a''$ are in $\aff(e)$. Let $J_{a'',a'}$ be the indicator that $a''\neq a'$. If 
\begin{align*}
\pr_e^e(a')& + \lambda I_a\pr_e^a(e') + \lambda I_{a'} \pr_e^{a'}(e)
\\\geq&\pr_e^e(a) + \lambda I_a\pr_e^{a}(e) + \lambda I_{a'}\pr_e^{a'}(e'') + \lambda I_{a''}J_{a'',a'}\pr_e^{a''}(e'),
\end{align*}
then $e$ cannot prefer $\mu'$ to $\mu$.
\end{enumerate}
\end{lem}

\begin{proof}
For 1:
\begin{align*}
\agg_a(\mu') =& \pr_a(e) + \sum_{e^*\in \mu'(a)\setminus e} \pr_a(e^*)
\\\leq& \pr_a(e') + \sum_{e^*\in \mu(a)\setminus e'} \pr_a(e^*)\tag{1}\label{line:prefs1}
\\=&\agg_a(\mu),
\end{align*}
where line~\ref{line:prefs1} comes from the fact that the two summations sum over the same matches of $a$, and $\pr_a(e) \leq \pr_a(e')$. This completes the first part of the Lemma. We will now show 2, for $b_1,\ldots,b_{|\aff(a)|}\in\aff(a)$:
\begin{align*}
\agg_e&(\mu') \\=& \pr_e^e(a) + \sum_{a^*\in\mu'(e)\setminus\{a\}} \pr_e^e(a^*) + \lambda I_{a} \left(\pr_e^{a}(e) + \sum_{e^*\in\mu'(a)\setminus\{e\}} \pr_e^{a}(e^*)\right) 
\\&+ \lambda I_{a'} \left(\pr_e^{a'}(e'') + \sum_{e^*\in\mu'(a')\setminus\{e''\}} \pr_e^{a'}(e^*)\right) \\&+\lambda  I_{a''}J_{a'',a'} \left(\pr_e^{a''}(e') + \sum_{e^*\in\mu'(a'')\setminus\{e'\}} \pr_e^{a''}(e^*)\right) 
\\&+ \lambda \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in \mu'(a^*)} \pr_e^{a^*} (e^*)
\\\leq& \pr_e^e(a') + \sum_{a^*\in\mu(e)\setminus\{a'\}} \pr_e^e(a^*) + \lambda I_{a} \left(\pr_e^{a}(e') + \sum_{e^*\in\mu(a)\setminus\{e'\}} \pr_e^{a}(e^*)\right) 
\\&+ \lambda I_{a'} \left(\pr_e^{a'}(e) + \sum_{e^*\in\mu(a')\setminus\{e\}} \pr_e^{a'}(e^*)\right) \\&+\lambda  I_{a''}J_{a'',a'} \left(\sum_{e^*\in\mu(a'')} \pr_e^{a'}(e^*)\right) 
\\&+ \lambda \sum_{a^*\in \aff(e)\setminus\{a,a',a''\}} \sum_{e^*\in\mu(a^*)}\pr_e^{a^*} (e^*)\tag{2}\label{line:prefs2}
\\=& \agg_e(\mu)
\end{align*}
where line~\ref{line:prefs2} comes from the fact that all the summations are over the same matches, and otherwise the terms we pull out compose the provided inequality. When we pull out the summation for $a''$, note that this is only something we can pull out if $a''\neq a'$, because otherwise we already pulled it out as the $a'$ summation. This is why we scale it by $J_{a'',a'}$.
\end{proof}

We now introduce another useful lemma that implies that any potential blocking tuple with a nontrivial $a''$ cannot be a blocking tuple. Thus we can simplify the potential blocking tuples we consider to find blocking tuples.


\begin{lem}\label{lem:tup}
Let $\mu$ be the resulting matching from \textsf{PriorityMatch}. Then any blocking tuple $\T = (a,a',a'',e,e',e'')$ must satisfy $a'' = a'$ or $a'' \in \mathcal{E}$.
\end{lem}

\begin{proof}
Assume for contradiction there exists a blocking tuple where $a''\notin \mathcal{E}\cup \{a'\}$. Since $a$ prefers $\mu'$, Lemma~\ref{lem:prefs} implies that $\pr_a(e') = 0$. But since $(a,e')$ is a match, they must have been present in some graph. The only possible graph is $G_4$. Since they were both matched in $G_4$, that means $e'$ had unfilled quota in all previous matchings. Now we consider $a''$. Because this is a blocking tuple, we know $\mu'\setminus\{(a'',e')\} \prec_{a''} \mu'$ and $\mu'\setminus\{(a'',e')\} \prec_{e'}^f \mu'$. Obviously, this means $a''$ and $e'$ must both have an interest in $(a'',e')$: $\pr_{a''}(e') = 1 $ and either $\pr_{e'}^{e'}(a'')= 1$ or $a'' \in \aff(e')$ and $\pr_{e'}^{a''}(e') = 1$. In both cases, $(a'',e')$ appeared as an edge sometime before $G_4$. We already showed that $e'$ cannot have met its quota during the processing of the graph where $(a'',e')$ appears, and neither could $a''$ because it never meets its quota. Thus they should have been matched by \textsf{PriorityMatch}. This contradicts the definition of the blocking tuple.
\end{proof}

We now prove the lemma defining when \prm{} works.

\begin{proof}[Proof of Lemma~\ref{lem:prior}]
Obviously, as the quotas always reflect the maximum remaining space any agent has for  matches, this creates a valid matching. We now show this is stable.

Consider $\mu$, the output of \textsf{PriorityMatch} that satisfies what we call the \textit{preconditions} of this lemma. Specifically, for any potential blocking tuple $\mathcal{T} = (a,a',a'',e,e',e'')$ such that $a,a'\in\aff(e)$ and $a$ prefers the swapped matching of $\mu$ with respect to $\mathcal{T}$, then:

\[\pr_e^e(a') + \lambda\pr_e^a(e') + \lambda\pr_e^{a'}(e) \geq \pr_e^e(a) +  \lambda\pr_e^a(e) + \lambda\pr_e^{a'}(e''). \tag{1}\label{eq:precond}\]

By Lemma~\ref{lem:tup}, we can ignore the $a''$ parameter as it will be either the same as $a'$ or in $\mathcal{E}$. Thus our tuple is effectively reduced to $\mathcal{T} = (a,a',e,e',e'')$. Assume for contradiction that $\mathcal{T}$ is a blocking tuple. Let $\mu'$ be the swapped matching of $\mu$ with respect to $\mathcal{T}$. Note that to use Inequality~\ref{eq:precond}, it is sufficient to show that $a,a'\in \aff(e)$ and $\mu \succ_a \mu'$ (i.e., the precondition of the lemma). The latter is satisfied because we assume $\T$ is a blocking tuple. Additionally, this would imply that $I_a=I_{a'}=1$, which yields (also due to the fact that $J_{a'',a'}=0$ by Lemma~\ref{lem:tup}):

\begin{align*}
 \pr_e^e(a')& + \lambda I_a\pr_e^a(e') + \lambda I_{a'} \pr_e^{a'}(e)
\\\geq&\pr_e^e(a) + \lambda I_a\pr_e^{a}(e) + \lambda I_{a'}\pr_e^{a'}(e'') + \lambda I_{a''}J_{a'',a'}\pr_e^{a''}(e'),
\end{align*}

This satisfies the second inequality of Lemma~\ref{lem:prefs}, which implies $e$ cannot prefer $\mu'$ to $\mu$. This is a contradiction. Therefore, any time we can prove or assume $a,a'\in\aff(a)$, we immediately get a contradiction. When we refer to this, we will simply cite the precondition.

Now, for $a$ and $e$ to form the blocking tuple, each must have some degree of interest $\mu'$ according to Lemma~\ref{lem:prefs}. This means $\pr_a(e) = 1$. For $e$, since it prefers $\mu'$, then at least one of the following must be true: $\pr_e^e(a)=1$, $a\in\aff(e)$ and $\pr_e^a(e)=1$, or $a'\in\aff(e)$ and $\pr_e^{a'}(e'')=1$. Again, we don't need to consider $a''$ because of Lemma~\ref{lem:tup}. We now do a case by case analysis based off of affiliations and preferences (note that we say $\mu_i$ is the maximal matching found by \prm{} in $G_i$):

\begin{enumerate}
\item\label{agg0} If $a\in\aff(e)$, $\pr_e^e(a) =1$, and $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_0$. Since it wasn't matched, $a$ or $e$ must have reached its quota without matching to the other. This is impossible for $a$ because it can only have an edge to $e$ in $G_0$. Thus, $e$ reached its quota in $G_0$ without matching to $a$. That means $(a',e)$ was matched across by $\mu_0$, which implies that $a'\in\aff(e)$. Since $a,a'\in \aff(e)$, we reach a contradiction due to our precondition.

\item Else if $a\in\aff(e)$ and $\pr_e^e(a) =1$ exclusively or $\pr_e^a(e)=1$: Then $(a,e)$ is an edge in $G_2$ or $G_3$. Since they weren't matched, that means either $a$ or $e$ met its capacity beforehand, by $\mu_0$, $\mu_1$, $\mu_2$, or $\mu_3$. If it was $a$, then $a$ and $e'$ were matched in one of these matchings, so $\pr_a(e')=1$. Then by Lemma~\ref{lem:prefs}, $a$ cannot prefer $\mu'$. This is a contradiction.

Otherwise, we do an analysis of the right and lefthand sides of the 2nd Lemma~\ref{lem:prefs} inequality. We can assume $a'\notin\aff(e)$, otherwise we get our contradiction from the precondition. Thus $I_{a'}=0$. We also know that in this case $\pr_e^e(a)=1$ exclusively or $\lambda \pr_e^a(e)=\lambda \leq 1$, and as always $J_{a'',a'}=0$. Therefore, the righthand side becomes:
\[\pr_e^e(a) + \lambda I_a\pr_e^{a}(e) + \lambda I_{a'}\pr_e^{a'}(e'') + \lambda I_{a''}J_{a'',a'}\pr_e^{a''}(e') \leq 1\]
And on the left, note that since $e$ and $a'$ must have matched before $(e,a)$ appeared in $G_3$ (so they matched in $\mu_0$, $\mu_1$, $\mu_2$, or $\mu_3$), then $\pr_e^e(a') = 1$ or $I_{a'}\pr_e^{a'}(e)=1$. We know the latter is not true since $I_{a'}=0$, thus $\pr_e^e(a')=1$. This gives:
\[\pr_e^e(a') + \lambda I_a\pr_e^a(e') + \lambda I_{a'} \pr_e^{a'}(e) \geq 1 + I_a\pr_e^a(e')  \geq 1 \]
Clearly the second term is at least as large as the first, implying $e$ does not prefer $\mu'$ to $\mu$, a contradiction.

\item Else if $a\in\aff(e)$ and $\pr_a(e)=0$ or $\pr_e^e(a)=\pr_e^a(e)=0$: The former is an immediate contradiction by the first inequality of Lemma~\ref{lem:prefs}. If the latter is true, then the entire righthand size of the second inequality of Lemma~\ref{lem:prefs} is 0, so we again get the same contradiction.

\item Else if $a' \in \aff(e)$, $\pr_e^e(a') = 1$, and $\pr_e^{a'}(e) = 1$: Again, we know from our precondition that $I_a=0$ (else, $a,a'\in\aff(e)$). Since $J_{a'',a'}=0$, the righthand side of the Lemma~\ref{lem:prefs} second inequality is at most:
\[\pr_e^e(a) + \lambda I_a\pr_e^{a}(e) + \lambda I_{a'}\pr_e^{a'}(e'') + \lambda I_{a''}J_{a'',a'}\pr_e^{a''}(e') \leq 1+\lambda\]
On the left, the assumptions for this case immediately yield (since $I_{a'}=1$):
\[\pr_e^e(a') + \lambda I_a\pr_e^a(e') + \lambda I_{a'} \pr_e^{a'}(e) = 1 + \lambda\]

Thus the second inequality of Lemma~\ref{lem:prefs} holds, yielding our contradiction that $e$ cannot prefer $\mu'$ to $\mu$.

\item Else if $a'\in\aff(e)$ and $\pr_e^e(a') = 1$ exclusively or $\pr_e^{a'}(e)=1$: Then $(a',e)$ is an edge in $G_2$ or $G_3$. That means $e$ could not have met its quota before $G_2$. On the other hand, $a\notin\aff(e)$ by our precondition, so $(a,e)$ could only appear in $G_1$, if at all. Since $a$ and $e$ were not matched, either $a$ met its quota in or before $G_1$, or $(a,e)$ was not in $G_1$. The former is a contradiction because it would imply $\pr_a(e')=1$ because they were matched early, but $a$ prefers $\mu'$ (Lemma~\ref{lem:prefs}, Inequality 1). The latter similarly implies $\pr_a(e)=0$, which would mean $a$ cannot prefer $\mu'$ (a contradiction), or $e$ has no interest in $a$, so $\pr_e^e(a)=0$. Now we look again to the second inequality in Lemma~\ref{lem:prefs}. On the right, most of the terms drop out since $\pr_e^e(a)=I_a=J_{a'',a'}=0$:
\[\pr_e^e(a) + \lambda I_a\pr_e^{a}(e) + \lambda I_{a'}\pr_e^{a'}(e'') + \lambda I_{a''}J_{a'',a'}\pr_e^{a''}(e') \leq \lambda\]
On the left, either the first or third term remains, giving us the following bound:
\[\pr_e^e(a') + \lambda I_a\pr_e^a(e') + \lambda I_{a'} \pr_e^{a'}(e) \geq \lambda\]
Thus we get the same contradiction.

\item Else if $a'\in \aff(e)$: At this point, $\pr_e^e(a') =0$ and $\pr_e^{a'}(e) = 0$. Thus $(a',e)$ could not have been in $G_0$, $G_1$, or $G_2$ because $e$ has no interest in $a'$. However, it cannot be present in another graph either since $a'\in\aff(e)$. This contradicts that $(a',e)$ were matched at all.

\item Else: Either $(a,e)$ is an edge in $G_1$, $\pr_a(e)=0$, or $\pr_e^e(a) = 0$. If $(a,e)$ is an edge in $G_1$, that means one of $a$ or $e$ was matched to their quota in $\mu_0$ or $\mu_1$. The former implies $\pr_a(e')=1$ because they were matched by $\mu_0$ or $\mu_1$, which is a contradiction by Lemma~\ref{lem:prefs}, inequality 1. Otherwise, if it were $e$, then the only possibility is that $(a',e)$ was in $G_1$, which means, $\pr_e^e(a')=1$. This implies the lefthand side of the second inequality of Lemma~\ref{len:prefs} is at least 1. Since $I_a=I_{a'}=J_{a'',a'}=0$, the righthand side is at most one. This satisfies the inequality and gives our contradiction.

Otherwise, if $\pr_a(e)=0$, then $a$ cannot prefer $\mu'$ by the first inequality of Lemma~\ref{lem:prefs}. If $\pr_e^e(a)=0$, then the righthand side of the second inequality of Lemma~\ref{lem:prefs} is zero, which again gives us the contradiction.
\end{enumerate}
Thus we have contradicted the possibility of having a blocking tuple, so our algorithm produces a stable marriage.
\end{proof}


Finally, we prove the weakness of \textsf{PriorityMatch} in the prioritized setting.


\begin{proof}[Proof of Lemma~\ref{lem:bad}]
Consider a market with two agents on each side: $A=\{a_1,a_2\}$ and $E=\{e_1,e_2\}$. We let $\aff(e_1) = \{a_1,a_2\}$ and $\aff(e_2) = \emptyset$. All possible preferences are set to one \textit{except} $\pr_{e_1}^{a_2}(e_2) = 0$, $\pr_{e_2}^{e_2}(a_2)=0$, and $\pr_{a_2}(e_2) = 0$. All quotas are 1. This means that $G_0$ contains edges $(a_1,e_1)$ and $(a_2,e_1)$. Since $e_1$ has a quota of 1, it must select only one edge. In an arbitrary maximal matching, it might select $(a_1,e_1)$. All other graphs, at this point, will either be empty, or only have edges with at least one 0-quota endpoint. Thus $a_2$ and $e_2$ will not be matched (though, we could imagine just arbitrarily matching the rest at the end and our argument will hold). However, note that $a_2$ likes $e_1$ and dislikes $e_2$. Similarly, $e_1$ would prefer for its affiliate $a_1$ to be matched with $e_2$ than $a_2$ be matched with $e_2$. Clearly, $a_2$ and $e_1$ would prefer to be matched and allow $a_1$ and $e_2$ to be matched. 
\end{proof}
